Efficient Guided Generation for Large Language Models

In this article we show how the problem of neural text generation can be constructively reformulated in terms of transitions between the states of a finite-state machine. This framework leads to an efficient approach to guiding text generation with regular expressions and context-free grammars by allowing the construction of an index over a language model's vocabulary. The approach is model agnostic, allows one to enforce domain-specific knowledge and constraints, and enables the construction of reliable interfaces by guaranteeing the structure of the generated text. It adds little overhead to the token sequence generation process and significantly outperforms existing solutions. An implementation is provided in the open source Python library Outlines

==> math-commands.tex <==
%
% Basic math commands
%
% brandonwillard@gmail.com
% (some material originally borrowed from Thomas Minka)
%
\RequirePackage{mathtools}

%\usepackage{xifthen}
\let\D\relax
\DeclareMathOperator*{\D}{D}
\let\H\relax
\DeclareMathOperator*{\H}{H}
\DeclareMathOperator*{\prox}{prox}
%\newcommand{\prox}[2] {
%  \ensuremath{
%    \operatornamewithlimits{prox}_{#1}\ifthenelse{\equal{#2}{}}{}{\left(#2\right)}
%  }
%}
\newcommand*{\moreau}[2]{
  \ensuremath{
    {#2}^{
    \ifx&#1&\empty 1 \else #1 \fi
    }
    %{#2}^{\ifthenelse{\equal{#1}{}}{1}{#1}}
  }
}

\newcommand*{\jac}[1]{
  \ensuremath{ \operatornamewithlimits{J}_{#1}
  }
}


\DeclareMathOperator{\dom}{dom}
\newcommand{\var}{{\rm var}}
\newcommand{\Tr}{^{\rm T}}
\newcommand{\rmlog}{\rm log}
\newcommand{\vtrans}[2]{{#1}^{(#2)}}
\newcommand{\kron}{\otimes}
\newcommand{\schur}[2]{({#1} | {#2})}
\newcommand{\schurdet}[2]{\left| ({#1} | {#2}) \right|}
\newcommand{\had}{\circ}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\invdiag}{\diag^{-1}}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\nullsp}{null}
\DeclareMathOperator{\tr}{tr}
\renewcommand{\vec}{\operatorname{vec}}
\DeclareMathOperator{\vech}{vech}
\renewcommand{\det}[1]{\left| #1 \right|}
\newcommand{\pdet}[1]{\left| #1 \right|_{+}}
\newcommand{\pinv}[1]{#1^{+}}
\DeclareMathOperator{\erf}{erf}
\newcommand{\hypergeom}[2]{\operatorname{{}_{#1}F_{#2}}}

% boldface characters
\renewcommand{\a}{{\bf a}}
\renewcommand{\b}{{\bf b}}
\renewcommand{\c}{{\bf c}}
\renewcommand{\d}{{\rm d}}  % for derivatives
\newcommand{\e}{{\bf e}}
\newcommand{\f}{{\bf f}}
\newcommand{\g}{{\bf g}}
\newcommand{\h}{{\bf h}}
%\newcommand{\k}{{\bf k}}
% in Latex2e this must be renewcommand
\renewcommand{\k}{{\bf k}}
\newcommand{\m}{{\bf m}}
\newcommand{\n}{{\bf n}}
\renewcommand{\o}{{\bf o}}
\newcommand{\p}{{\bf p}}
%\newcommand{\q}{{\bf q}}
\renewcommand{\r}{{\bf r}}
\newcommand{\s}{{\bf s}}
\renewcommand{\t}{{\bf t}}
\renewcommand{\u}{{\bf u}}
\renewcommand{\v}{{\bf v}}
\newcommand{\w}{{\bf w}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
%\newcommand{\z}{{\bf z}}
\newcommand{\A}{{\bf A}}
\newcommand{\B}{{\bf B}}
%\newcommand{\C}{{\bf C}}
%\newcommand{\D}{{\bf D}}
\newcommand{\E}{{\bf E}}
\newcommand{\F}{{\bf F}}
%\newcommand{\G}{{\bf G}}
%\renewcommand{\H}{{\bf H}}
\newcommand{\I}{{\bf I}}
\newcommand{\J}{{\bf J}}
\newcommand{\K}{{\bf K}}
%\renewcommand{\L}{{\bf L}}
\newcommand{\M}{{\bf M}}
\newcommand{\Nor}{{\cal N}}  % for normal density
%\newcommand{\N}{{\bf N}}
\renewcommand{\O}{{\bf O}}
\renewcommand{\P}{{\bf P}}
\newcommand{\Q}{{\bf Q}}
\newcommand{\R}{{\bf R}}
\renewcommand{\S}{{\bf S}}
\newcommand{\T}{{\bf T}}
%\newcommand{\U}{{\bf U}}
\newcommand{\V}{{\bf V}}
\newcommand{\W}{{\bf W}}
\newcommand{\X}{{\bf X}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\Z}{{\bf Z}}

\renewcommand{\Re}{{\mathbb{R}}}

% this is for latex 2.09
% unfortunately, the result is slanted - use Latex2e instead
%\newcommand{\bfLambda}{\mbox{\boldmath$\Lambda$}}
% this is for Latex2e
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}

% Yuan Qi's boldsymbol
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
%\newcommand{\Beta}{\boldsymbol{\eta}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bnabla}{\boldsymbol{\nabla}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda}{\mathbf{\Lambda}}

\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}

\newcommand{\bgamma}{\mathbf{\gamma}}
\newcommand{\bGamma}{\mathbf{\Gamma}}

\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bPsi}{\mathbf{\Psi}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\1}{{\bf 1}}
\newcommand{\0}{{\bf 0}}

%\newcommand{\comment}[1]{}

\newcommand{\bs}{\backslash}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\notS}{{\backslash S}}
\newcommand{\nots}{{\backslash s}}
\newcommand{\noti}{{\backslash i}}
\newcommand{\notj}{{\backslash j}}
\newcommand{\nott}{\backslash t}
\newcommand{\notone}{{\backslash 1}}
\newcommand{\nottp}{\backslash t+1}
% \newcommand{\notz}{\backslash z}

\newcommand{\notk}{{^{\backslash k}}}
%\newcommand{\noti}{{^{\backslash i}}}
\newcommand{\notij}{{^{\backslash i,j}}}
\newcommand{\notg}{{^{\backslash g}}}
\newcommand{\wnoti}{{_{\w}^{\backslash i}}}
\newcommand{\wnotg}{{_{\w}^{\backslash g}}}
\newcommand{\vnotij}{{_{\v}^{\backslash i,j}}}
\newcommand{\vnotg}{{_{\v}^{\backslash g}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\quart}{\frac{1}{4}}
\newcommand{\msgb}{m_{t \leftarrow t+1}}
\newcommand{\msgf}{m_{t \rightarrow t+1}}
\newcommand{\msgfp}{m_{t-1 \rightarrow t}}

\newcommand{\proj}[1]{\operatorname{proj}\negmedspace\left[#1\right]}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\DeclareMathOperator{\dif}{d}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\DeclareMathOperator{\N}{N}

\newcommand{\Rbar}{ \overline{\R} }
\newcommand{\sgn}{\mathop{\mathrm{sgn}}}

\newcommand{\vnorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\enorm}[1]{\Vert #1 \Vert_2}

%\newcommand{\norm}{\mathcal{N}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cK}{\mathcal{K}}

\newcommand{\tN}{\tilde{N}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tF}{\tilde{F}}

\newcommand{\bx}{{\bf x}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\bX}{{\bf X}}
\newcommand{\by}{{\bf y}}
\newcommand{\IG}{\mathcal{IG}}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\lhat}[1][i]{\hat\lambda_{#1}^{-1(g)}}
\newcommand{\what}[1][j]{\hat\omega_{#1}^{-1(g)}}
\newcommand{\bone}{{\bf 1}}
\newcommand{\Li}{\hat\Lambda^{-1(g)}}
\newcommand{\Oi}{\hat\Omega^{-1(g)}}
\newcommand{\iid}{\stackrel{\mathrm{iid}}{\sim}}
\newcommand{\iidp}{\stackrel{\mathrm{P}}{=}}
\newcommand{\iidd}{\stackrel{\mathrm{D}}{=}}
% NOTE: requires mathtools package
\newcommand{\defeq}{\coloneqq}

\newtheorem{exa}{Example}
\newtheorem{definition}{Definition}
%\newtheorem{theorem}{\bf Theorem}
%\newtheorem{Proof}{Proof}
%\numberwithin{Def}{section}
%\newtheorem{remark}{\bf Remark}
%\newtheorem{Qes}{Question}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{\bf Lemma}
%\newtheorem{Cor}{\bf Corollary}
%\numberwithin{Cor}{section}
%\newtheorem{Eq}{Equation}[section]

